Towards Realistic Example-based Modeling via 3D Gaussian Stitching

Using parts of existing models to rebuild new models, commonly termed as example-based modeling, is a classical methodology in the realm of computer graphics. Previous works mostly focus on shape composition, making them very hard to use for realistic composition of 3D objects captured from real-world scenes. This leads to combining multiple NeRFs into a single 3D scene to achieve seamless appearance blending. However, the current SeamlessNeRF method struggles to achieve interactive editing and harmonious stitching for real-world scenes due to its gradient-based strategy and grid-based representation. To this end, we present an example-based modeling method that combines multiple Gaussian fields in a point-based representation using sample-guided synthesis. Specifically, as for composition, we create a GUI to segment and transform multiple fields in real time, easily obtaining a semantically meaningful composition of models represented by 3D Gaussian Splatting (3DGS). For texture blending, due to the discrete and irregular nature of 3DGS, straightforwardly applying gradient propagation as SeamlssNeRF is not supported. Thus, a novel sampling-based cloning method is proposed to harmonize the blending while preserving the original rich texture and content. Our workflow consists of three steps: 1) real-time segmentation and transformation of a Gaussian model using a well-tailored GUI, 2) KNN analysis to identify boundary points in the intersecting area between the source and target models, and 3) two-phase optimization of the target model using sampling-based cloning and gradient constraints. Extensive experimental results validate that our approach significantly outperforms previous works in terms of realistic synthesis, demonstrating its practicality. More demos are available at https://ingra14m.github.io/gs_stitching_website.

==> table/per-scene-VQA.tex <==
\begin{tabular}{r|cc|cc|cc|cc|cc}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{LIVE\_VQC} & \multicolumn{2}{c|}{KoNViD-1k} & \multicolumn{2}{c|}{LSVQ\_Test} & \multicolumn{2}{c|}{LSVQ\_1080P} & \multicolumn{2}{c}{YouTube\_UGC} \\
                  & $\Delta t \uparrow$              & $\Delta a \uparrow$             & $\Delta t \uparrow$              & $\Delta a \uparrow$             & $\Delta t \uparrow$              & $\Delta a \uparrow$              & $\Delta t \uparrow$               & $\Delta a \uparrow$              & $\Delta t \uparrow$               & $\Delta a \uparrow$              \\ \hline
case1             & \badcolor{-0.075}              & \goodcolor{+0.149}             & \badcolor{-0.058}              & \goodcolor{+0.142}             & \badcolor{-0.049}              & \goodcolor{+0.140}              & \badcolor{-0.059}               & \goodcolor{+0.148}              & \badcolor{-0.066}               & \goodcolor{+0.094}              \\
case2             & \goodcolor{+0.887}              & \goodcolor{+0.453}             & \goodcolor{+0.804}              & \goodcolor{+0.394}             & \goodcolor{+0.760}              & \goodcolor{+0.376}              & \goodcolor{+0.808}               & \goodcolor{+0.442}              & \goodcolor{+0.841}               & \goodcolor{+0.413}              \\
case3             & \goodcolor{+0.057}              & \goodcolor{+0.326}             & \goodcolor{+0.052}              & \goodcolor{+0.284}             & \goodcolor{+0.049}              & \goodcolor{+0.270}              & \goodcolor{+0.052}               & \goodcolor{+0.318}              & \goodcolor{+0.054}               & \goodcolor{+0.298}              \\
case4             & \goodcolor{+0.706}              & \badcolor{-0.337}             & \goodcolor{+0.640}              & \badcolor{-0.293}             & \goodcolor{+0.605}              & \badcolor{-0.278}              & \goodcolor{+0.642}               & \badcolor{-0.327}              & \goodcolor{+0.669}               & \badcolor{-0.307}              \\
case5             & \goodcolor{+0.077}              & \goodcolor{+0.078}             & \goodcolor{+0.070}              & \goodcolor{+0.067}             & \goodcolor{+0.066}              & \goodcolor{+0.064}              & \goodcolor{+0.070}               & \goodcolor{+0.075}              & \goodcolor{+0.073}               & \goodcolor{+0.070}              \\
case6             & \goodcolor{+0.370}              & \goodcolor{+0.051}             & \goodcolor{+0.335}              & \goodcolor{+0.044}             & \goodcolor{+0.317}              & \goodcolor{+0.043}              & \goodcolor{+0.337}               & \goodcolor{+0.050}              & \goodcolor{+0.351}               & \goodcolor{+0.047}              \\
case7             & \goodcolor{+0.528}              & \goodcolor{+0.132}             & \goodcolor{+0.478}              & \goodcolor{+0.115}             & \goodcolor{+0.454}              & \goodcolor{+0.109}              & \goodcolor{+0.482}               & \goodcolor{+0.129}              & \goodcolor{+0.501}               & \goodcolor{+0.121}              \\
case8             & \goodcolor{+0.018}              & \badcolor{-0.179}             & \goodcolor{+0.016}              & \badcolor{-0.156}             & \goodcolor{+0.015}              & \badcolor{-0.148}              & \goodcolor{+0.016}               & \badcolor{-0.174}              & \goodcolor{+0.017}               & \badcolor{-0.163}              \\
case9             & \goodcolor{+1.053}              & \goodcolor{+0.426}             & \goodcolor{+0.953}              & \goodcolor{+0.372}             & \goodcolor{+0.902}              & \goodcolor{+0.355}              & \goodcolor{+0.957}               & \goodcolor{+0.416}              & \goodcolor{+0.997}               & \goodcolor{+0.390}              \\
case10             & \goodcolor{+0.887}              & \badcolor{-0.039}             & \goodcolor{+0.804}              & \badcolor{-0.033}             & \goodcolor{+0.761}              & \badcolor{-0.032}              & \goodcolor{+0.807}               & \badcolor{-0.037}              & \goodcolor{+0.841}               & \badcolor{-0.035}              \\
case11             & \goodcolor{+0.284}              & \goodcolor{+0.018}             & \goodcolor{+0.257}              & \badcolor{-0.022}             & \goodcolor{+0.244}              & \goodcolor{+0.012}              & \goodcolor{+0.259}               & \badcolor{-0.027}              & \goodcolor{+0.269}               & \badcolor{-0.014}              \\
case12             & \goodcolor{+0.072}              & \badcolor{-0.293}             & \goodcolor{+0.065}              & \badcolor{-0.256}             & \goodcolor{+0.062}              & \badcolor{-0.242}              & \goodcolor{+0.065}               & \badcolor{-0.285}              & \goodcolor{+0.068}               & \badcolor{-0.268}              \\
case13             & \goodcolor{+0.349}              & \badcolor{-0.120}             & \goodcolor{+0.317}              & \badcolor{-0.104}             & \goodcolor{+0.299}              & \badcolor{-0.099}              & \goodcolor{+0.318}               & \badcolor{-0.116}              & \goodcolor{+0.331}               & \badcolor{-0.109}              \\
case14             & \goodcolor{+0.459}              & \goodcolor{+0.014}             & \goodcolor{+0.416}              & \badcolor{-0.012}             & \goodcolor{+0.392}              & \goodcolor{+0.011}              & \goodcolor{+0.417}               & \goodcolor{+0.014}              & \goodcolor{+0.435}               & \badcolor{-0.013}              \\
case15             & \goodcolor{+0.101}              & \badcolor{-0.426}             & \goodcolor{+0.092}              & \badcolor{-0.371}             & \goodcolor{+0.087}              & \badcolor{-0.353}              & \goodcolor{+0.092}               & \badcolor{-0.415}              & \goodcolor{+0.097}               & \badcolor{-0.390}              \\
case16             & \goodcolor{+0.040}              & \goodcolor{+0.091}             & \goodcolor{+0.036}              & \goodcolor{+0.079}             & \goodcolor{+0.034}              & \goodcolor{+0.076}              & \goodcolor{+0.036}               & \goodcolor{+0.089}              & \goodcolor{+0.038}               & \goodcolor{+0.082}              \\
case17             & \goodcolor{+0.053}              & \badcolor{-0.014}             & \goodcolor{+0.048}              & \goodcolor{+0.012}             & \badcolor{-0.015}              & \goodcolor{+0.012}              & \badcolor{-0.028}               & \goodcolor{+0.014}              & \badcolor{-0.050}               & \badcolor{-0.013}              \\
case18             & \goodcolor{+0.386}              & \goodcolor{+0.117}             & \goodcolor{+0.349}              & \goodcolor{+0.101}             & \goodcolor{+0.330}              & \goodcolor{+0.097}              & \goodcolor{+0.350}               & \goodcolor{+0.114}              & \goodcolor{+0.366}               & \goodcolor{+0.107}              \\
case19             & \goodcolor{+0.019}              & \badcolor{-0.205}             & \goodcolor{+0.017}              & \badcolor{-0.178}             & \goodcolor{+0.016}              & \badcolor{-0.170}              & \goodcolor{+0.017}               & \badcolor{-0.199}              & \goodcolor{+0.018}               & \badcolor{-0.187}              \\
case20             & \badcolor{-0.088}              & \badcolor{-0.091}             & \badcolor{-0.079}              & \badcolor{-0.079}             & \badcolor{-0.075}              & \badcolor{-0.075}              & \badcolor{-0.081}               & \badcolor{-0.089}              & \badcolor{-0.083}               & \badcolor{-0.083}              \\
case21             & \goodcolor{+0.022}              & \badcolor{-0.031}             & \goodcolor{+0.019}              & \badcolor{-0.027}             & \goodcolor{+0.018}              & \badcolor{-0.015}              & \goodcolor{+0.020}               & \badcolor{-0.030}              & \goodcolor{+0.021}               & \badcolor{-0.018}              \\ 
average             & \goodcolor{+0.295} & \goodcolor{+0.006} & \goodcolor{+0.268} & \goodcolor{+0.004} & \goodcolor{+0.251} & \goodcolor{+0.007} & \goodcolor{+0.266} & \goodcolor{+0.005} & \goodcolor{+0.276} & \goodcolor{+0.001}              \\ \hline
\end{tabular}
